Enhanced Boundary Learning for Glass-like Object Segmentation

Glass-like objects such as windows, bottles, and mirrors exist widely in the real world. Sensing these objects has many applications, including robot navigation and grasping. However, this task is very challenging due to the arbitrary scenes behind glass-like objects. This paper aims to solve the glass-like object segmentation problem via enhanced boundary learning. In particular, we first propose a novel refined differential module that outputs finer boundary cues. We then introduce an edge-aware point-based graph convolution network module to model the global shape along the boundary. We use these two modules to design a decoder that generates accurate and clean segmentation results, especially on the object contours. Both modules are lightweight and effective: they can be embedded into various segmentation models. In extensive experiments on three recent glass-like object segmentation datasets, including Trans10k, MSD, and GDD, our approach establishes new state-of-the-art results. We also illustrate the strong generalization properties of our method on three generic segmentation datasets, including Cityscapes, BDD, and COCO Stuff. Code and models is available at \url{https://github.com/hehao13/EBLNet}.

==> 3method_bak.tex <==
 \section{Method}
% logits
%  Problem of existing approaches
%  Our proposed methods
%   1, Refined Differential Module
%   2, Edge-aware point based GCN
%   3, Cascade / Loss(Constructive Loss)


\begin{figure}[!t]
	\centering
	\includegraphics[scale=0.35]{fig/network.pdf}
	\caption{
	\small Cascade Network Architecture. We adopt DeeplabV3+ for illustration where the RDM and PGM are connected in a cascaded order. Best view it on screen and zoom in.
	}
	\label{fig:network}
\end{figure}

In this section, we will first give a detailed description of our proposed Refined Differential Module~(RDM) used to generate the precise edge and segmentation results. Inputs of RDM are $F_{low}, F_{refine}$ and $F_{in}$, which are low-level features of backbone, the relative high-level feature of backbone and outputs of other modules, respectively. Outputs of RDM are segmentation features and boundary prediction denoted as $F_{merge}$ and $F_{b}$. Then, to use precise boundary prediction $F_b$ as a guidance to help the  global edge feature learning and generate more accurate segmentation result in the final output. The edge-aware Point-based Graph convolution network Module~(PGM) is proposed to enforce consistency on boundaries. Inputs of PGM are the outputs of RDM and the outputs of PGM are refined segmentation feature $F'_{merge}$ used to generate the final prediction. Finally, we will detail the generalized cascaded network architecture and loss function design, respectively. Network architecture is shown in Fig.~\ref{fig:network}.


\subsection{Refined Differential Module}

\noindent \textbf{Motivation and overview:} Our motivation consists of two aspects: Firstly, to generate the fine-grained edges $F_{b}$, low-level features $F_{low}$ provide detailed positional cues for edge prediction proven in previous work~\cite{deeplabv3p,kirillov2019pointrend}. We use it to refine feature $F_{in}$ with high semantics for better edge prediction. Secondly, directly predicting the edges using low-level details may involve much noise, particularly for the glass-like objects where the inner content changes various for different scenes. Motivated by residual edge prediction in traditional image processing~\cite{evans2006morphological}, we adopt a residual learning strategy to sharpen the edge features $F_{edge}$ from the inner of the object using direct supervision from ground truth masks. 

In general, the first step is to obtain edge-aware feature $F_{edge}$ with direct edge supervision where the low-level feature $F_{low}$ is extra input. The second step is to obtain better residual feature representation, which generates more accurate edge prediction with direct residual supervision. We use a refine feature $F_{refine}$ as extra input in this step. \iffalse Since edge prediction of first step may not be very accurate, some vital features for residual part may be removed after subtraction operation, we use a fine-grained feature $F_{refine}$ as extra input in this step.\fi Finally, both edge and residual features are added together to generate $F_{merge}$ which serves as the input for the next module or output. The whole process is shown in Fig.~\ref{fig:RDE}(a). Since there are two refinements and one subtraction operation, we name our module Refined Differential Module or RDM for short. 

\begin{figure}[!t]
	\centering
	\includegraphics[width=0.8\linewidth]{fig/RDM.pdf}
	\caption{
	\small (a) Refined Differential Module, $L_{edge}$ and $L_{residual}$ are losses of edge part prediction and residual part prediction. (b) Feature visualization comparison. The second and the third column represent the edge feature $F_{edge}$ before and after using fine-grained edge prediction. After using fine-grained edge prediction, the edge feature $F_{edge}$ is more discriminative. Best view it on screen and zoom in.
	}
	\label{fig:RDE}
\end{figure}

\noindent \textbf{Coarse Edge Prediction with Edge Supervision:}  Given the input feature $F_{in} \in \RR^{H \times W \times C}$, rather than predicting edge using input feature $F_{in}$ only, we refine $F_{in}$ with low-level feature $F_{low}$. First, $F_{low}$ is resized into the $F_{in}$ size bilinearly, then $F_{low}$ and $F_{in}$ are concatenated together, after that a $3\times3$ convolution layer is used to fuse features and reduce the number of channels. This process can be formulated as Equ.~\ref{equ:coarse_edge_predition}, after this process, we obtain the edge features $F_{edge}$.  With $F_{edge}$, another two $3\times3$ convolution layer is used as segmentation head to generate edge prediction $F_b$ supervised by a binary edge map. Then the residual (non-edge) feature $F_{residual}$ is generated using Equ.~\ref{equ:subtraction}. 

\begin{equation}
F_{edge} = Conv(Concat(F_{low}, F_{in}))
\label{equ:coarse_edge_predition}
\end{equation}
\begin{equation}
    F_{residual} = F_{in} - F_{edge}
    \label{equ:subtraction}
\end{equation}

\noindent \textbf{Fine-grained Edge Prediction with Residual Learning:}
Our motivations have two folds: (1) For the glass-like objects, the inner part may bring noises for edge prediction. Better feature representation of the residual part will make it easier to learn a better edge around the glass-object. (2) Since edge-aware feature $F_{edge}$ of the first step may not be very accurate, the subtraction operation may remove some vital features for $F_{residual}$. So we adopt another fine-grained feature $F_{refine}$ generated from the backbone to get refined $F'_{residual}$ for better residual learning. The residual learning performs similar roles as dilation in morphological processing~\cite{papari2011edge} to make the inner part grow up towards edge part, then the subtraction leads to thinner boundaries. Thus with residual learning on residual parts, $F_{edge}$ will shrink into thinner representation, which is beneficial to generate better edge features. The prediction $F_r$ of residual part is generated using another two $3\times3$ convolution layers. The total process of the second step is shown in Equ.~\ref{equ:refine residual} and Equ.~\ref{equ:coarse_edge_predition_learning}:
\begin{equation}
	F'_{residual} = Conv(Concat(F_{residual}, F_{refine}))
	\label{equ:refine residual}
\end{equation}
\begin{equation}
F_{r} = Conv(F'_{residual})
\label{equ:coarse_edge_predition_learning}
\end{equation}
 $F_{r}$ is supervised by cross-entropy loss with the same as the final prediction. Finally, we add $F'_{residual}$ and ${F}_{edge}$ as the merged feature $F_{merge}$ for following processing.

To best show the effect of our module, we give the feature visualization on $F_{edge}$ for both coarse edge prediction and fine-grained edge prediction with residual learning in Fig.~\ref{fig:RDE}(b) by performing PCA on $F_{edge}$ into 3 dimensions for visualization. Compared to only supervises the edge part, joint supervision on both edge and residual part can produce more accurate edge features, which supports our motivation for edge sharpening via residual learning.
 \iffalse Compared with ground truth mask, our methods lead to more precise and thinner boundary results than those with only edge supervision.\fi
 
\subsection{Edge-aware Point-based GCN}

\begin{figure}[!t]
	\centering
	\includegraphics[width=0.8\linewidth]{fig/pointGCN.pdf}
	\caption{
	\small Proposed Point-based Graph convolution Module(PGM). (a) shows several failure cases for dense affinity learning in DAnet~\cite{DAnet}, selected points are marked red. For the first and the second images, the red point is on the glass, while its affinity map mainly comes from the bottle not the glass. For the third and the fourth images, the affinity map of the red point does not come from the glass to which it belongs. (b) describes the pipeline of PGM. (c) proves the effectiveness of PGM. After using PGM, the boundary is much smoother and more consistent. Best view it on screen and zoom in.
	}
	\label{fig:pointGCN}
\end{figure}

After obtaining the fine-grained edge prediction $F_b$, we further propose an efficient Point-based Graph Convolution Network (GCN) that uses $F_b$ as a guidance to help $F_{merge}$ generate more accurate final predictions, especially on the boundaries.

\noindent \textbf{Limitation of Graph Convolution Network:} Graph convolution~\cite{gcnpaper} is a highly efficient and differentiable module that allows long-range information exchange in a single layer.
This is done by defining edges $\mathbb{E}$ among nodes $\mathbb{V}$ in a graph $\mathbb{G}$. Formally, the graph convolution is defined as
\begin{equation}\label{eq:gcn}    
\tilde{\mathbf{X}} =  \sigma(\mathbf{W} \mathbf{X} \mathbf{A}),
\end{equation}
where $\sigma(\cdot)$ is the non-linear activation function, $\mathbf{A}\in \mathbb{R}^{N\times N}$ is the adjacency matrix characterising the neighbourhood relations of the graph, $\mathbf{X}$ is the input features and $\mathbf{W}\in\mathbb{R}^{D \times \tilde{D}}$ is the weight matrix. Non-local networks~\cite{non_local,DAnet,EMAnet} can be viewed as a fully connected graphical model. However, the full image grid affinity can not be learned well on glass-like objects. It may bring noise into transparent objects due to the change of the various backgrounds or inner parts besides its huge computation and memory cost. Take DANet~\cite{DAnet} as an example, we visualize the spatial affinity from its head by selecting pixels of glass objects. As shown in Fig.~\ref{fig:pointGCN}(a), the inner parts can not provide the context cues to support the final prediction.

Rather than applying GCN on the whole image grids~\cite{DAnet} or projection space~\cite{SGR_gcn} as in previous work, we propose to apply GCN on point-wised features on $F_{merge}$ to enhance the representation. We name this module as Point-based GCN Module or PGM.


\noindent \textbf{Point-Based Graph Convolution Network on Edge:} Fig~\ref{fig:pointGCN}(b) shows the pipeline of PGM. Given edge prediction $F_b$ and merged feature $F_{merge}$, we need to build the point node graph $G$ , which has $K$ point features sampled from $F_{merge}$ according to the confidence score in $F_b$. Specifically, we first sample at most $K$ points with the highest confidence in $F_{b}$. Then, we use indexes of these sampled points to sample the according $K$ point features from $F_{merge}$. \iffalse and sample top-$K$ points from $F_{merge}$ with the coordinates in $b$. \fi Finally with these sampled features, we build the input point graph $G_{in} \in K\times C $. We adopt the same settings in GCN~\cite{gcnpaper} for information diffusion. A simple choice of $\mathbf{A}$ is a $1 \times 1$ convolutional layer that can be updated by the general backpropagation and make the whole model can be trained end to end. Similar to the previous works~\cite{beyond_grids,glore_gcn}, we consider adopting a Laplacian matrix $\left( \mathbf{I} - \mathbf{A}_{g} \right)$ to propagate the node features over the graph, where the identity matrix $\mathbf{I}$ serves as a residual sum connection.

\begin{equation}
\mathbf{G}_{out} = \sigma \left( \mathbf{W}_{g} \mathbf{G}_{in} \left(\mathbf{I} - \mathbf{A}_{g} \right)\right),
\label{eq:gcn1}
\end{equation}

After reasoning, we replace the point features in $G_{out}$ into $F_{merge}$ according to their indexes as the final feature representation $F'_{merge}$. PGM is efficient and effective in handling glass-like transparent objects since the global edge information is essential to improve the discrimination power of the network. As shown in Fig.~\ref{fig:pointGCN}(c), after PGM, the final segmentation boundary is smoother and more consistent.
%according t the ground truth mask. 

\subsection{Network Architecture and Loss function}

In this section, we will give a detailed description of network architecture and loss function design.

\noindent \textbf{Cascade Refined Decoder} Cascade refinement has been proven effective for various learning tasks such as Cascade R-CNN~\cite{cascade_rcnn} and RefineNet~\cite{refinenet}. For each stage, we take the output of PGM $F'_{merge}$ as the new input $F_{in}$ for the next stage RDM while the $F_{refine}$ is designed by introducing different stages feature from the backbone network. $F'_{merge}$ is used to generate the prediction $F_m$ of merge part using a segmentation head consisted of three convolutional layers. As the low-level features are essential for detecting object boundaries, we add $F_{low}$ as input for every stage. We use the $F_{m}$ of the last cascade layer as the final output. Since our proposed modules are lightweight, cascaded learning does not lead to much computation cost during the inference while contributes to a significant gain on final results. 

\noindent \textbf{Network Architecture} Fig.~\ref{fig:network} illustrates the whole network architecture, which bases on the state-of-the-art model DeeplabV3+~\cite{deeplabv3p}. Here we utilize dilated ResNet as backbone~\cite{resnet,dilation} only for illustration purpose. The output stride of backbone is 8 in our experiment unless otherwise specified. Our proposed module is inserted after the ASPP module~\cite{deeplabv3p}, the output feature of ASPP module is served as the first input $F_{in}$. Our method can be easily extended to other methods~\cite{fcn,pspnet,DAnet} which can be found in the experiment part. 

\noindent \textbf{Loss function Design} There are three different prediction results at each cascade stage, namely $F_b$, $F_r$, $F_m$, which are predictions of edge part, residual part and merge part, respectively. We define a joint loss function shown in Equ.~\ref{equ:joint_loss}.
\begin{equation}
    \label{equ:joint_loss}
    \begin{aligned}
    L_{joint} = &\lambda_{1}L_{residual}(F_r, G_r) + \lambda_{2}L_{edge}(F_b, G_e) + \\ &\lambda_{3}L_{merge}(F_m, G_m)
    \end{aligned}
\end{equation}
 $G_m$ represents the original ground truth, the ground truth of edge part $G_e$ generated from $G_m$ is a binary edge mask with thickness 8. When generating the ground truth of residual part $G_r$ the corresponding position of the positive pixel of $G_e$ in $G_r$ is marked as ignore and the other pixels of $G_r$ are the same as $G_m$. 
$\lambda_1$, $\lambda_2$ and $\lambda_3$ are hyper-parameters which balance the importance between $L_{residual}, L_{edge}$ and $L_{merge}$ and we set $\lambda_1=1, \lambda_2=3, \lambda_3=1$ in our experiments. $L_{merge}$ and $L_{residual}$ are standard Cross-Entropy(CE) Loss. $L_{edge}$ is Dice Loss~\cite{DiceLoss}. Since our network is a cascade paradigm, the final loss function is addition of each stage, formulated as $ L=\sum_{n=1}^{N}L_{joint}^{n} $, where $N$ represents the number of cascade layer.
